Discretization Drift in Two-Player Games

Gradient-based methods for two-player games produce rich dynamics that can solve challenging problems, yet can be difficult to stabilize and understand. Part of this complexity originates from the discrete update steps given by simultaneous or alternating gradient descent, which causes each player to drift away from the continuous gradient flow -- a phenomenon we call discretization drift. Using backward error analysis, we derive modified continuous dynamical systems that closely follow the discrete dynamics. These modified dynamics provide an insight into the notorious challenges associated with zero-sum games, including Generative Adversarial Networks. In particular, we identify distinct components of the discretization drift that can alter performance and in some cases destabilize the game. Finally, quantifying discretization drift allows us to identify regularizers that explicitly cancel harmful forms of drift or strengthen beneficial forms of drift, and thus improve performance of GAN training.

==> explicit_regularization.tex <==
\section{Connection to explicit regularizers}

The form of the modified losses that we have derived are related to explicit regularizers to stabilize adversarial training of GANs.
Consensus optimization, SGDA, ODE-GAN and \citep{nagarajan2017gradient} are introducing explicit regularization to reduce the strength
of the rotational field of the game or to stabilize training. While the form of the modified losses we introduce are similar, our use of explicit regularization is only as a form to understand the effect of the implicit regularizers that we have found, rather than solving the aformentioned issues in GAN training. Cancelling the effect of implicit gradient regularization is not sufficient, as can be seen by ODE-GAN, which still requires a regularizer despite not having first order regularization effects. The arguments regarding the rotational field of the underlying game remain regardless of the integrator used - something that would need to be further analysed in the light of the implicit regularization we have derived. We are making statements about the effect of discretization on the underlying two player game, and notice its effects, rather than make statements about what regularization is required given the underlying game. We should also make the difference between penaltizes which minimise your own norm, or penaltize which minimise the norm of the other player - like discussed in ~\citep{nagarajan2017gradient}, there is a connection there with unrolled gans and increased stability.


The comparison between different methods is shown in Table~\ref{tab:methods_comp}.

\begin{table*}[h]
\centering
\begin{tabular}{ |c|c|c| }
 \hline
 Method & Discriminator ($\phi$) & Generator ($\theta$)\\
 \hline
 \hline
 IGR (A) & $- \frac {\alpha h}{4m}\norm{\nabla_{\phi} E}^2 + \frac{\alpha h}{4}\norm{\nabla_{\theta} E}^2$ & $ \frac{(2 \alpha - \lambda) h}{4}\norm{\nabla_{\phi} E}^2 + \frac{\lambda h}{4k}\norm{\nabla_{\theta} E}^2$  \\
 IGR (S) & $-h/4\norm{\nabla_{\phi} E}^2 + h/4\norm{\nabla_{\theta} E}^2$  & $-h/4\norm{\nabla_{\phi} E}^2 + h/4\norm{\nabla_{\theta} E}^2$ \\
 SGA/ACO (S) \citep{balduzzi2018mechanics} & - $\eta sign(\nabla_{\phi} E,\nabla_{\phi}\norm{\nabla_{\phi} E}^2) \norm{\nabla_{\phi} E}^2$ &  $\eta sign(\nabla_{\phi} E,\nabla_{\theta}\norm{\nabla_{\theta} E}^2) \norm{\nabla_{\theta} E}^2$ \\
 Consensus opt (S)\citep{mescheder2017numerics} & $-\eta \norm{\nabla_{\phi} E}^2 - \eta \norm{\nabla_{\theta} E}^2$ & $\eta \norm{\nabla_{\phi} E}^2 + \eta \norm{\nabla_{\theta} E}^2$ \\
Locally stable GAN (S) \citep{nagarajan2017gradient} & \text{\sffamily X} &  $\eta \norm{\nabla_{\phi} E}^2$ \\
 ODE-GAN (S)& $ - \eta \norm{\nabla_{\theta} E}^2$ &  \text{\sffamily X} \\
 \hline
\end{tabular}
\caption{Comparison with different methods in the zero sum case. We assume a $\min_{\theta} \max_{\phi}$ game, so we translate signs from the other papers (in case they use a min min or max max formulation). The learning rates assumed are $\alpha h$ and $\lambda h$ for the discriminator and generator, and the number of updates $m$ and $k$, respectively. S and A denote whether updates are simultaneous or alternating.}
\label{tab:methods_comp}
\end{table*}


Beyond this, add here a few other related works.

